A Direct Approach to Multi-class Boosting and Extensions

Boosting methods combine a set of moderately accurate weaklearners to form a highly accurate predictor. Despite the practical importance of multi-class boosting, it has received far less attention than its binary counterpart. In this work, we propose a fully-corrective multi-class boosting formulation which directly solves the multi-class problem without dividing it into multiple binary classification problems. In contrast, most previous multi-class boosting algorithms decompose a multi-boost problem into multiple binary boosting problems. By explicitly deriving the Lagrange dual of the primal optimization problem, we are able to construct a column generation-based fully-corrective approach to boosting which directly optimizes multi-class classification performance. The new approach not only updates all weak learners' coefficients at every iteration, but does so in a manner flexible enough to accommodate various loss functions and regularizations. For example, it enables us to introduce structural sparsity through mixed-norm regularization to promote group sparsity and feature sharing. Boosting with shared features is particularly beneficial in complex prediction problems where features can be expensive to compute. Our experiments on various data sets demonstrate that our direct multi-class boosting generalizes as well as, or better than, a range of competing multi-class boosting methods. The end result is a highly effective and compact ensemble classifier which can be trained in a distributed fashion.

==> CVPR2011/alg.tex <==
%
%
%
%
\SetKwInput{KwInit}{Initilaize}
\SetVline
\linesnumbered

\begin{algorithm}[t]
\caption{\multiboost with the hinge loss.
}
\begin{algorithmic}
%\normalsize{
%\small{
%\scriptsize{
   \KwIn{
   % \begin{itemize}
   %    \item

     1)    A set of examples $\{\bx_i,y_i\}$, $i=1 \cdots m$;
   %
   %   \item
     $
     \;
     $
     \\2)    The maximum number of weak classifiers, $T$;
   %\end{itemize}
   }

   \KwOut{
% \begin{itemize}
%    \item
      A multi-class classifier $F(\bx) = \argmax_r \sum_{j=1}^{T} w_{r,j} h_j(\bx)$;
%\end{itemize}
}

\KwInit {

   % \begin{itemize}
   %    \item
   1)      $t \leftarrow 0$;
   %   \item
   \\2)      Initialize sample weights, $U = 1/k$;
   %\end{itemize}
}

\While{ $t < T$ }
{
  1) Find the weak classifier by solving the subproblem \eqref{EQCVPR11:sub1};
  \\2) If the stopping criterion has been met, we exit the loop.\\
   \If{ 
   $ \sum_{i=1}^m \left[ \delta_{r,y_i} - U_{ir} \right] h(\bx_i) 
    < \nu  + \epsilon $ } { break; }
  3) Add the best weak classifier, $h_t(\cdot)$, into the primal problem;
  \\4) Solve the primal problem \eqref{EQCVPR11:P1} using
       a primal-dual interior-point LP solver such as  \citet{mosek},
       such that
       the dual solution is also available.
  \\5) $t \leftarrow t + 1$;
}

%} % End \small
%
\end{algorithmic}
\label{ALGCVPR11:alg1}
\end{algorithm}




==> CVPR2011/fig_cal.tex <==
% LaTeX Source
% Author:        Chunhua Shen {chhshen@gmail.com}
% Creation:      Friday 12/11/2010 00:06.
% Last Revision: Monday 24/01/2011 00:04.



\begin{figure*}[tp!]
\setlength{\fboxsep}{1pt}
\setlength{\fboxrule}{1pt}
%cartman
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0001}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0004}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0013}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0019}}
 \includegraphics[width = 0.25cm,height = 0.85cm]{white}
%headphones
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0002}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0009}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0010}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0022}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0024}}
 \includegraphics[width = 0.25cm,height = 0.85cm]{white}
%iris
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0004}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0031}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0037}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0048}}
 \includegraphics[width = 0.25cm,height = 0.85cm]{white}
%paperclip
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0025}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0044}}
 \includegraphics[width = 0.25cm,height = 0.85cm]{white}
%skunk
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0005}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0017}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0025}}
 \colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0027}}
% another row
% cartman
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0030}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0050}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0080}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{032_0090}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%headphones
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0036}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0045}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0057}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0080}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0115}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%iris
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0080}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0082}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0091}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0102}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%paperclip
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0058}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0073}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%skunk
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0037}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0064}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0078}}
\colorbox{green}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0081}}
% blank row
%\includegraphics[width = 0.85\textwidth,height = 0.05cm]{white}
% misclassified
%\vspace{.0001 mm}
%{\rule{\linewidth}{0.5mm}}
%cartman
\\
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0013}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0093}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0068}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0050}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%headphones
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0013}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0033}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0064}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0087}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{186_0071}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%iris
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0037}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0010}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0028}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0042}}
\includegraphics[width = 0.3cm,height = 0.85cm]{white}
%paperclip
\includegraphics[width = 0.52cm,height = 0.85cm]{white}
\includegraphics[width = 0.52cm,height = 0.85cm]{white}
\includegraphics[width = 0.5cm,height = 0.85cm]{white}
%skunk
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{101_0019}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{118_0038}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0082}}
\colorbox{red}{\includegraphics[width = 0.52cm,height = 0.85cm]{155_0092}}
   \caption{
   Some examples of correctly classified (top two rows) and misclassified (bottom row)
   images by \mbh.
   The categories are ``{cartman}'', ``{headphones}'', ``{iris}'',
   ``{paperclip}'' and ``{skunk}''.
   The accuracy of this test is $71.2\%$.
   No image is falsely classified into the category of ``{paperclip}''.
   }
\label{figCVPR11:cal-samples}
\end{figure*}



==> CVPR2012/ADMM.tex <==
%
%
%
%
\SetKwInput{KwInit}{Initilaize}
\SetVline
\linesnumbered

\begin{algorithm}[t]
\caption{ADMM for solving \eqref{EQCVPR12:logPrimalL12}}
\begin{algorithmic}
%\normalsize{
%\small{
%\scriptsize{
   \KwIn{

     1)    Outputs of weak classifiers, $H$;
     $ \; $
     \\2)    Augmented Lagrangian parameter, $\lambda$;
     $ \; $
     \\3)    The maximum number of iterations, $s_{\rm max}$;
   }

   \KwOut{
      An optimal $W^{\ast}$;
   }

\KwInit {

   1)      $s \leftarrow 0$;
   $ \; $
   \\2)      $W^{0}$, $Z^{0}$, $U^{0}$;
}

\Repeat{ {\rm convergence}}
{
  $W^{s+1} = \argmin_{W} \frac{1}{mk} \sum_{i=1}^m
        \sum_{r=1}^k \log\bigl(1+\exp\left( - \rho_{ir} \right)\bigr)+
 %   $
 %  \\      $\quad \quad \quad \quad 
 %  
  (U^s)^\T W + \frac{\lambda}{2} \| W - Z^s \|_2^2 $;
  \\ Update $Z_{j:}^{s+1} $ using \eqref{EQCVPR12:ADMM8};
  % $Z_{j:}^{s+1} = \mathcal{S}_{\lambda/\rho}(W_{j:}^{s+1} + U_{j:}^{s}), \forall j$
  % where $\mathcal{S}_\kappa(a) = (1 - \kappa/\| a \|_2)_{+}a$;
  \\ $U^{s+1} = U^s + \lambda ( W^{s+1} - Z^{s+1} )$;
  \\ $s \leftarrow s + 1$;
  \\   \If{ $s > s_{\rm max}$ } { break; }
}

%} % End \small
%
\end{algorithmic}
\label{ALG:ADMM}
\end{algorithm}







==> CVPR2012/alg.tex <==
%
%
%
%
\SetKwInput{KwInit}{Initilaize}
\SetVline
\linesnumbered

\begin{algorithm}[t]
\caption{MultiBoost with shared weak classifiers via group sparsity.
%
%{\bf
%MODIFY THIS PART to make all the notation/symbols consistent with
%those in the text!
%}
}
\begin{algorithmic}
%\normalsize{
%\small{
%\scriptsize{
   \KwIn{
   % \begin{itemize}
   %    \item

     1)    A set of examples $\{\bx_i,y_i\}$, $i=1 \cdots m$;
   %
   %   \item
     $
     \;
     $
     \\2)    The maximum number of weak classifiers, $T$;
   %\end{itemize}
   }

   \KwOut{
% \begin{itemize}
%    \item
      A multi-class classifier $F(\bx) = \argmax_r \sum_{j=1}^{T} w_{r,j} h_j(\bx)$;
%\end{itemize}
}

\KwInit {

   % \begin{itemize}
   %    \item
   1)      $t \leftarrow 0$;
   %   \item
   \\2)      Initialize sample weights, $U_{ir} = 1/(mk)$;
   %\end{itemize}
}

\While{ $t < T$ }
{
  1) Train a weak learner,
  $h_t(\cdot) = $
  $$
  \left\{ \begin{array}{ll}
  \argmax_{h(\cdot) \in \mathcal{H},r}  \sum_{i=1}^m
  \left[
  \delta_{r,y_i}  - U_{ir}
   \right] h(\bx_i) , &\mbox{{hinge loss}} \\
  \argmax_{h(\cdot),r}  \sum_{i=1}^m
  \left[
  \delta_{r,y_i} \left( \textstyle \sum_{l} U_{il} \right) - U_{ir}
   \right] h(\bx_i) , &\mbox{{logistic}}
       \end{array} \right.
  $$
   %$\forall r, \forall h(\cdot) \in \mathcal{H}$;
  \\2) If the stopping criterion has been met, we exit the loop.\\
   \If{ $\Bigl\| \sum_{i=1}^m \left[
   \delta_{r,y_i} - U_{ir}
   \right] h(\bx_i) \Bigr\|_2
    < \nu  + \epsilon $ } { break; \quad {(hinge loss)}}
     \If{ $\Bigl\| \sum_{i=1}^m \left[
   \delta_{r,y_i} \left( \textstyle \sum_{l} U_{il} \right) - U_{ir}
   \right] h(\bx_i) \Bigr\|_2
    < \nu  + \epsilon $ } { break; \quad {(logistic loss)}}
  3) Add the best weak learner, $h_t(\cdot)$, into the current set;
  \\4) Solve either the primal or the dual problem (we solve the dual \eqref{EQCVPR12:hinge7})
  for the { hinge loss case};
       or solve the primal problem \eqref{EQCVPR12:logPrimalL12} using \ADMM
  for the logistic loss case;
  \\5) Update sample weights (dual variables);
  \\6) $t \leftarrow t + 1$;
}

%} % End \small
%
\end{algorithmic}
\label{ALGCVPR12:alg1}
\end{algorithm}






